Nonlinear Model Predictive Control of a 3D Hopping Robot: Leveraging Lie Group Integrators for Dynamically Stable Behaviors

Achieving stable hopping has been a hallmark challenge in the field of dynamic legged locomotion. Controlled hopping is notably difficult due to extended periods of underactuation combined with very short ground phases wherein ground interactions must be modulated to regulate global state. In this work, we explore the use of hybrid nonlinear model predictive control paired with a low-level feedback controller in a multi-rate hierarchy to achieve dynamically stable motions on a 3D hopping robot. In order to demonstrate richer behaviors on the manifold of rotations, both the planning and feedback layers must be designed in a geometrically consistent fashion; therefore, we develop the necessary tools to employ Lie group integrators and appropriate feedback controllers. We experimentally demonstrate stable 3D hopping, as well as trajectory tracking and flipping in simulation.

==> Sections/Preliminaries.tex <==
\section{Preliminaries}
\subsection{Hybrid System Dynamics}
Hopping consists of alternating sequences of continuous and discrete dynamics; therefore, it is naturally modeled as a hybrid system. We begin by introducing the configuration of the hopping robot as $\b q = (\b p, \quat, \b \theta,  \ell)\in\mathcal{Q}$, where $\b p\in\R^3$ is the Cartesian position, $\quat\in S^3$ is the unit quaternion representing the orientation, $\b \theta\in\R^3$ represents the flywheel angles, and $\ell\in\R$ is the foot deflection. 
% With an abuse of notation, let $\dot q = (\b v, \b \omega, \dot{\b \theta},\dot{ \ell}) \in \R^3\times \mathfrak{s}^3\times \R^3\times \R$
Next, let $\b v = (\dot{\b p}, \b \omega, \dot{\b \theta},\dot{ \ell})\in \mathcal{V}\triangleq \R^3\times \mathfrak{s}^3\times \R^3\times \R$; then, the complete robot state can be written as $\b x = (\b q,\b v) \in \mathcal{X} \triangleq \mathcal{Q}\times \mathcal{V}$. Two distinct continuous phases of dynamics exist for the hopping robot, the \textit{flight} phase $f$ when the robot is in the air, and the \textit{ground} phase $g$ when the foot is contacting the floor. We can construct a directed graph with vertices $v\in V\triangleq\{f, g\}$ and edges $e \in E\triangleq\{f\to g, g\to f\}$ to characterize how the robot traverses the hybrid modes, as shown in \figref{fig:HybridGraph}. 

For each vertex $v\in V$, let $\mathcal{D}_v$ represent the admissible domain in which the system state evolves, and $n_v$ denote the number of holonomic constraints restricting the motion of the robot. Note that $n_f=0$, and $n_g = 3$, which pin the foot to the ground. Temporarily omitting the details for manifold value variables, which can be found in \cite{please_I_hope_there_is_a_reference_for_this}, let $\b J_v:\mathcal{Q}\to \R^{n_v \times n}$ denote the Jacobian of the holonomic constraints where $n = |\mathcal{Q}|$. We can define the dynamics as:
\begin{align*}
    % \b D(\b q)\ddot{\q} + \b H(\q, \dot{\q}) &= \b B \b u + \b J^\top_v(\q) \b \lambda_v \\ 
    % \dot{\b J\hspace{1pt}}_v(\q) \dot {\q} + \b J_v(\q) \ddot {\q} &= \b 0.
    \b D(\b q)\ddot{\b q} + \b H(\q, \dot{\q}) &= \b B \b u + \b J^\top_v(\q) \b \lambda_v \\ 
    \dot{\b J\hspace{1pt}}_v(\q) \dot {\q} + \b J_v(\q) \ddot {\q} &= \b 0.
\end{align*}
where $\b D:\mathcal{Q}\to \mathbb{R}^{n\times n}$ is the mass-inertia matrix, $\b H:\mathcal{X}\to \mathbb{R}^n$ contains the Coriolis and gravity terms, $\b B\in\mathbb{R}^{n\times m}$ is the actuation matrix, $\b u \in \mathbb{R}^m$ is the control input, and $\b \lambda_v\in \R^{n_v}$ are the Lagrange variables describing the constraint forces. These equations can be rearranged and forces $\b \lambda_v$ solved for in order to produce the constraint implicit dynamics:
\begin{align*}
    % \dot{\b x} = \b f_{v}(\b x) + \b g_{v}(\b x)\b u.  % We do not use control affine form, and the exposition is clearer without it.
    \dot{\b x} = \b f_{v}(\b x, \b u),
\end{align*}
% where $\b f_v:\mathcal{X}\to \mathbb{R}^{2n}$ and $\b g_v:\mathcal{X}\to \mathbb{R}^{2n\times m}$ are the drift vector and actuation matrix in the domain $v$, respectively. 
where $\b f_v:\mathcal{X}\to \mathbb{R}^{2n}$ is of control-affine form. 

% \triangleq \R^3\times S^3\times \R^3\times \R$
%  \in \mathcal{Q}

% The domain $\mathcal{D}_v$ encodes reasonable system states (for example the robot being above the floor), as well as the various .

% as well as the $n_v$ holonomic constraints restricting the motion of the robot.

% For each edge $e\in E$, let $s(e)$ denote the source vertex and $t(e)$ the target edge. A hybrid transition occurs when the system state intersects the \textit{guard}, defined as: 
% $$\mathcal{S}_{s(e)} = \{\b x \in \mathcal{D}_{s(e)} ~|~ \b h_e(x) = 0, \dot{\b h}_e(x) < 0\},$$ 
% where $\b h_e:\mathcal{Q}\to \R$ is a function describing the impact condition. For the hopping robot, $\b h_{f\to g}$ is the vertical position of the foot, and $\b h_{g\to f} = \b\ell$, as shown in \figref{fig:HybridGraph}.

Each hybrid transition $e\in E$ occurs when the system state intersects the \textit{guard}, defined as: 
\begin{alignat*}{2}
    \mathcal{S}_{f} &= \{\b x \in \mathcal{D}_{f} ~|~ p_z(q) = 0, \dot{p}_z(x) < 0\}~~~&&e = f\to g,\\
    \mathcal{S}_{g} &= \{\b x \in \mathcal{D}_{g} ~|~ \ell = 0, \dot{\ell} < 0\}&&e = g\to f,
\end{alignat*}
where $p_z:\mathcal{Q}\to\R$ returns the vertical position of the foot. For an edge $e = v_1\to v_2$, upon striking the guard $\mathcal{S}_{v_1}$ the system undergoes a discrete jump in states as described by:
\begin{align*}
    \b x^+ = \b \Delta_e(\x^-) 
\end{align*}
where $\b \Delta_e : \mathcal{S}_{v_1} \to \mathcal{D}_{v_2}$ describes the momentum transfer though impact, and $\b x^-$ and $\b x^+$ are the pre and post-impact states, respectively. Collecting the various objects $\mathcal{D} = \{\mathcal{D}_v\}_{v\in V}$, $\mathcal{S}=\{\mathcal{S}_v\}_{v\in V}$, $\b\Delta = \{\b\Delta_e\}_{e\in E}$ and $FG=\{(\b f_v, \b g_v)\}_{v\in V}$, we are equipped to describe the hybrid control system of the hopping robot via the tuple:
\begin{align*}
    \mathcal{HC} = (V, E, \mathcal{D}, \mathcal{S}, \b\Delta, FG).
\end{align*}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/HopperDomains.pdf}
    \caption{The robot traversing the various hybrid domains.}
    \label{fig:HybridGraph}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=0.97\textwidth]{Figures/LieGroup2.pdf}
    \caption{A depiction of Lie groups, Lie algebras, and the $\log$ operation. a) The trajectory $\bar{\quat}_k$, b) pulling the trajectory back to the identity element via $\bar{\quat}_0^{-1}$, and c) taking the $\log$ map near identity to obtain elements in the Lie algebra. \red{update}.\vspace{-4mm}}
    \label{fig:LieGroup}
\end{figure*}




% When the robot impacts the ground, three additional holonomic constraints are enforced $\b h: \mathcal{Q} \to \R^3$.

% $\mathcal{S} = \{\b x \in \mathcal{X} ~|~ \b h(x) = 0,  \dot{\b h}(x) < 0\}$


\subsection{Lie Group Integrators}
\label{sec:linearization}
In this section, we restrict our attention to the orientation coordinates of the robot and discuss how to perform integration. As every other variable is a vector in Euclidean space, local approximations are straightforward to produce \cite{local_linearizations_from_dynamics}. We represent the orientation of the rigid body via a unit quaternion $\quat\in S^3 = \{\quat\in\mathbb{H}~|~\|\quat\| = 1\}$. As opposed to Euler angles, quaternions do not suffer from issues of singularities, and provide a straightforward interpolation method -- this will be important in constructing continuous time signals from the discrete points that MPC produces. 
% One advantage of using quaternions as opposed to Euler angles is that there is a straightforward way to interpolate between them -- this will be important in constructing continuous time signals from the discrete points that MPC produces. 
Quaternions and their associated quaternion multiplication define a Lie group structure on $S^3$, which will be key in preforming MPC in a geometrically consistent fashion. The angular rate of the body is given by an element of the associated Lie algebra $\omega\in\mathfrak{s}^3$, the tangent space of $S^3$ at the identity element $\quat_{\mathcal{E}},$ the elements of which are purely imaginary quaternions.
% Note that we will use the quaternion convention of $\quat=(w,\mathbf{p})$ with real part $w$ first followed by imaginary vector $\mathbf{p}$.

The time rate of change of a unit quaternion at a point $\quat$ is given by an element of the tangent space at $\quat$, i.e. $\dot \quat \in T_\quat S^3$. Given the angular rate of the body $\b\omega$, we can calculate $\dot \quat$ as:
\begin{align}
    \dot \quat = \quat\b\omega, \label{eqn:q_dot}
\end{align}
using standard quaternion multiplication. The above formula is possible since the tangent map of left multiplication by a quaternion is also given by left multiplication, mapping from the Lie algebra to the tangent space at $\quat$. 
\footnote{Often, the equation \eqref{eqn:q_dot} is reported as $\dot \quat = \frac{1}{2}\quat\b\omega$. This is because the isomorphism between $\b\omega \in \mathfrak{s}^3$ and $\mathbb{R}^3$ is given by $\phi(\b\omega) = \frac{1}{2}\b\omega$ if the generators of $\mathfrak{s}^3$ are taken to be the canonical basis of imaginary 3-vectors, which arises from the fact that the action of quaternions parameterized by a rotation angle $\theta$ on vectors rotates them by an angle of $2\theta$.}
%
Integrating equation \eqref{eqn:q_dot} results in:
\begin{align}
    \quat(t) = \quat(0)\exp(\b\omega(t))
\end{align}
where $\exp:\mathfrak{s}^3\to S^3$ is termed the exponential map and maps elements of the Lie algebra $\mathfrak{s}^3$ back to the Lie group $S^3$. This map is injective for imaginary quaternions with magnitude less than $\pi$; over this neighborhood, the inverse map is denoted $\log$. If instead of directly integrating we take a Lie-Euler step, the above expression becomes:
\begin{align}
\label{eqn:lieEuler}
    \quat_{k+1} = \quat_k\exp(\b\omega_k h)
\end{align}
for a (small) time step $h\in\R$. This is a simple example of a \textit{Lie group integrator}.

